TeleMoMa: A Modular and Versatile Teleoperation System for Mobile Manipulation

A critical bottleneck limiting imitation learning in robotics is the lack of data. This problem is more severe in mobile manipulation, where collecting demonstrations is harder than in stationary manipulation due to the lack of available and easy-to-use teleoperation interfaces. In this work, we demonstrate TeleMoMa, a general and modular interface for whole-body teleoperation of mobile manipulators. TeleMoMa unifies multiple human interfaces including RGB and depth cameras, virtual reality controllers, keyboard, joysticks, etc., and any combination thereof. In its more accessible version, TeleMoMa works using simply vision (e.g., an RGB-D camera), lowering the entry bar for humans to provide mobile manipulation demonstrations. We demonstrate the versatility of TeleMoMa by teleoperating several existing mobile manipulators - PAL Tiago++, Toyota HSR, and Fetch - in simulation and the real world. We demonstrate the quality of the demonstrations collected with TeleMoMa by training imitation learning policies for mobile manipulation tasks involving synchronized whole-body motion. Finally, we also show that TeleMoMa's teleoperation channel enables teleoperation on site, looking at the robot, or remote, sending commands and observations through a computer network, and perform user studies to evaluate how easy it is for novice users to learn to collect demonstrations with different combinations of human interfaces enabled by our system. We hope TeleMoMa becomes a helpful tool for the community enabling researchers to collect whole-body mobile manipulation demonstrations. For more information and video results, https://robin-lab.cs.utexas.edu/telemoma-web.

==> sections/6_demo.tex <==
\section{Intended Demonstration}
\label{s:demo}

We plan to demonstrate \methodname{} to the live audience at RSS'24 in two alternative (or parallel, depending on the available space) manners. In the first, we will provide a demo of our teleoperation system for mobile manipulators in simulation. RSS audience members could teleoperate two mobile manipulators in the simulator OmniGibson~\cite{li2023behavior} using VR controllers, keyboard, 3D mouse or our visual system, or combinations thereof such as vision and VR controllers. In our second demo, we will provide a remote teleoperation system for one of our mobile manipulators in our lab. This will test the intercontinental remote capabilities for teleoperation of \methodname{}. In the lab, one of our members will facilitate resets and help with technical issues. For both demos, if the participants give their permission, we will collect their demonstrations for multiple mobile manipulation tasks and make the dataset available after the conference. Finally, depending on the availability of a real world platform, we may be able to also demonstrate teleoperation of a robot on site. We are evaluating the feasibility of using one of the robots of our colleagues participating in Robocup 2024 in Eindhoven near the time of RSS, but this possibility has yet to be confirmed.
